Recorp: Receiver-Oriented Policies for Industrial Wireless Networks

Future Industrial Internet-of-Things (IIoT) systems will require wireless solutions to connect sensors, actuators, and controllers as part of high data rate feedback-control loops over real-time flows. A key challenge in such networks is to provide predictable performance and adaptability in response to link quality variations. We address this challenge by developing RECeiver ORiented Policies (Recorp), which leverages the stability of IIoT workloads by combining offline policy synthesis and run-time adaptation. Compared to schedules that service a single flow in a slot, Recorp policies share slots among multiple flows by assigning a coordinator and a list of flows that may be serviced in the same slot. At run-time, the coordinator will execute one of the flows depending on which flows the coordinator has already received. A salient feature of Recorp is that it provides predictable performance: a policy meets the end-to-end reliability and deadline of flows when the link quality exceeds a user-specified threshold. Experiments show that across IIoT workloads, policies provided a median increase of 50% to 142% in real-time capacity and a median decrease of 27% to 70% in worst-case latency when schedules and policies are configured to meet an end-to-end reliability of 99%.

==> abstract.tex <==
The next generation of Industrial Internet-of-Things (IIoT) systems will require wireless solutions to connect sensors, actuators, and controllers as part of high data rate feedback-control loops over real-time flows.
A key challenge in such networks is to provide predictable performance and adaptability in response to variations in link quality.
We address this challenge by developing \emph{REC}eiver \emph{OR}iented \emph{P}olicies (\pn), which leverages the stability of IIoT workloads to build a solution that combines offline policy synthesis and run-time adaptation.
Compared to schedules that service a single flow in a slot, \pn policies share slots among multiple flows by assigning a coordinator and a list of flows that may be serviced in the same slot.
At run-time, the coordinator will dynamically execute one of the flows depending on which flows the coordinator has already received.
The net effect of this strategy is that %a node can dynamically repurpose the retransmissions remaining after receiving the data of an incoming flow to service other incoming flows opportunistically.
%Therefore, 
the flows that are executed in a slot can be adapted in response to the variable link conditions observed at run-time.
A key feature of \pn is that it provides \emph{predictable performance}: a policy meets the end-to-end reliability and deadline constraints of flows as long as the quality of the used links exceeds a user-specified threshold.
Testbed experiments demonstrate that \pn can adapt more effectively than traditional scheduling approaches to variations in link quality.
When \pn policies and schedules are configured to meet the same end-to-end reliability target of 99\%,
testbed results show that for a data collection workload, \pn policies increase the network's real-time capacity by a factor of 1.96 times.
Retrospective analysis indicates that for the same experiment, the analytical performance guarantees also held.
Larger-scale multihop simulations show that across typical IIoT workloads, policies provided a median improvement of 1.63 to 2.44 times in real-time capacity as well as a median reduction of 1.45 to 2.43 times  in worst-case latency. 



==> introduction.tex <==
% !TEX root = main.tex
\section{Introduction}
\label{sec:introduction}

Industrial Internet-of-Things (IIoT) systems are gaining rapid adoption in process control industries such as oil refineries, chemical plants, and factories. 
Such systems require a versatile wireless alternative to wired networks to connect sensors, actuators, and controllers as part of feedback-control loops over multi-hop real-time flows. 
%Since communication delays and packet losses may lead to severe degradation in control performance or even control instability, it is critical to develop wireless solutions that provide reliable and real-time communication while tolerating variations in link quality. 
Since communication delays and packet losses may lead to severe degradation in control performance or even control instability, it is critical that wireless solutions provide reliable and real-time performance that can tolerate variations in link quality.

Protocol designers commonly assume that there is an inherent trade-off between building agile networks that can adapt to dynamics and building networks that provide predictable performance (e.g., \cite{duquennoy2015orchestra,rtqs,li2015incorporating,8401919}).
Indeed, this assumption holds for the state-of-the-art approaches that use Time Slotted Channel Hopping (TSCH) to build predictable wireless networks.
%Indeed, this assumption holds for the state-of-the-art approach to building predictable wireless networks that use Time Slotted Channel Hopping (TSCH).
% TSCH combines Time Division Multiple Access (TDMA) and channel-hopping in a multichannel mesh network to provide predictable performance, and can be analyzed using existing real-time schedulability analysis (e.g., \cite{conflictAwareLeastLaxityFirst,endToEndAnalysis}).
TSCH combines Time Division Multiple Access (TDMA) and channel-hopping in a multi-channel mesh network. 
TSCH provides predictable performance that can be analyzed using existing real-time schedulability analyses (e.g., \cite{conflictAwareLeastLaxityFirst,endToEndAnalysis}).
However, it is challenging for TSCH networks to adapt packet transmissions in response to packet losses since this requires reconstructing a global schedule (which is expensive).
%Recognizing this limitation, TSCH networks such as WirelessHART, combine contention-free dedicated slots that are used for real-time communication and shared slots that used for best-effort service.
%In this paper, we pose the question of whether there is a \emph{a fundamental trade-off between predictability and flexibility.}
%We will show that it is possible to build dynamic policies that provide predictable performance and locally adapt in response to packet losses.
In this paper, we call this conventional wisdom into question by developing   \emph{\textbf{D}ynamic \textbf{P}ull-based \textbf{P}olicy \textbf{S}ynthesis} (DPPS) -- a new paradigm for building wireless networks that use \emph{policies} to provide higher performance and agility than  scheduling approaches while maintaining predictable performance in spite of link dynamics.
%

\textbf{Schedules vs. Policies:} To better understand the fundamental differences between schedules and policies, 
let us start by considering an idealized scenario in which a clairvoyant oracle provides immediate and accurate feedback regarding the success or failure of packet transmissions.
% plant?, Ryan
A feedback control system that has a state-of-the-art scheduler as the controller and the oracle as the plant could be used to build schedules iteratively.
Initially, the scheduler would schedule several transmissions based on the workload of the system.
Then, the oracle would provide feedback indicating which transmissions have been successful.
Based on this feedback, the scheduler could proceed to schedule the transmissions in the next slot.
The feedback control system is both adaptive and provides predictable performance as existing real-time schedulability analyses may be readily applied.
The open question is whether we can replace the clairvoyant oracle with a realistic model of the network's behavior while retaining both  properties.

Existing scheduling frameworks adopt a \emph{deterministic} model: the transmission of a link is successful after it is scheduled for a fixed number of slots.
The number of retransmissions is usually tuned based on the worst-case link quality.
%A schedule specifies the fixed slot and channel for each transmission. 
Due to the determinism of the model, in each slot of the schedule, we precisely know the flows that have arrived at a node.
This property simplifies the development of techniques to analyze the performance of real-time flows.
However, enforcing determinism has a significant performance cost.
Consider the transmission of a flow over a link for which several slots are allocated in a schedule.
If the packet is relayed to the next hop without exhausting the allocated transmissions, the unused slots cannot be reused as such changes would require global agreement to avoid transmission conflicts.
This example illustrates the inability of scheduling approaches that build on deterministic models to achieve both flexibility and predictability simultaneously.
%to adapt to the  transmission failures and successes observed at run-time and the potentially significant performance penalty it introduces.

In contrast to prior work, we propose a \emph{probabilistic} model:
we replace the oracle by a link model that provides a lower bound on the likelihood of a successful transmission.
A consequence of using a probabilistic model is that it is no longer possible to ascertain precisely which flows that have arrived at a node.
We propose \emph{dynamic pull policies} to account for this uncertainty.
A policy is a sequence of pull operations that will be performed in a slot.
A pull operation is executed by a coordinator node that can dynamically request data (i.e., a \texttt{pull}, henceforth) from a list of  flows depending on the outcome of previous transmissions.
The flows pertaining to the list are determined offline during the construction of the policy and reflects the uncertainty of which flows have arrived at a node by a given slot.
At run-time, the coordinator requests the packet of the first flow in the service list from which it has not yet received the packet.
The ability of the coordinator to switch which flow it services at run-time without requiring a global agreement or introducing additional communication overhead is the essential property of dynamic pull policies.
We will show that dynamic policies simultaneously provide greater flexibility than traditional schedules in adapting to packet losses while maintaining predictable performance.
%The additional flexibility results in networks that have real-time capacity and reliability.


% The central contribution of this paper is -- \emph{\textbf{D}ynamic \textbf{P}ull-based \textbf{P}olicy \textbf{S}ynthesis} (DPPS) -- a new paradigm for building wireless networks that uses \emph{policies} to provide higher performance and agility than state-of-the-art scheduling approaches while maintaining predictable performance in spite of network dynamics.
% To illustrate the differences between schedules and policies, 
% At the core of our approach are \emph{dynamic pull policies} in which nodes dynamically request data from neighbors (i.e., a \texttt{pull}, henceforth) depending on their local state.
% Each node maintains a flag for each flow routed through it, which indicates whether the node has received a packet of an instance of a flow. 
% The key advantage of dynamic policies is that, at run-time, nodes can adapt their transmissions locally without having to reconstruct the global schedule (which is prohibitively expensive).
% We will show that dynamic policies provide greater flexibility than traditional schedules in adapting to packet losses which translates into higher real-time capacity and reliability.

\textbf{Practical Synthesis:}
The synthesis of dynamic policies, however, poses two critical challenges ---
scaling the policy synthesis procedure and analyzing the performance provided by policies as the quality of links varies.
Ideally, for policy synthesis to be practical, it should scale to moderate size networks (30 -- 40 nodes) and support tens of real-time flows (30 -- 50 flows).
The critical decision is how to balance the trade-off between the expressiveness of policies, the  performance improvements they provide, and the scalability of the synthesis procedure.
Cognizant of these trade-offs, we make two important design choices:
(1) We limit the expressiveness of policies to include only nodes pulling data from their neighbors depending on their local state.
Since the actions of a node do not depend on the state of other nodes, the probabilities of packets being forwarded across links of a multi-hop flow are independent. 
This property reduces the number of states maintained during synthesis since it is sufficient to capture the interactions of flows locally at each node rather than globally across the network.
(2) The synthesis procedure includes a \builder and an \evaluator.
Policies are built incrementally in a slot-by-slot manner using the feedback control approach we previously outlined. 
The \builder casts the problem of determining the pulls that will be performed in the current slot as an Integer Linear Program (ILP).
In turn, the evaluator applies the policy actions while tracking the system state as it evolves from slot to slot. The iterative nature of the synthesis procedure improves its scalability as it requires that we only maintain the states associated with the current slot.

\textbf{Reliability Model:}
To replace the clairvoyant oracle, we propose a Threshold Link Reliability (TLR) model that is based on the more general framework of parametric Markov Chains (MC). 
Our goal is  to guarantee that each flow has a minimum level of reliability not only for a specific link quality but for a wide range of possible values which capture the inherent variability of wireless links.
We model the quality of a link as a parameter $P_s$ that is lower-bounded by a user-specified minimum packet reception rate ($P_{m}$) such that $P_{m} \le P_s \le 1$.
%\footnote{Guidelines for deploying WirelessHART networks suggest that typical values of $P_m$ are in the range 60--70\%.}. 
The \evaluator uses symbolic algebraic manipulation to construct a polynomial $E_i$ that characterizes the end-to-end reliability of a flow $F_i$ as a function of $P_s$. 
% this is kind of misleading since it implies its always true.  We have proved it is true in some cases and conjecture it is true in the remaining.  I'm not sure how else to word this though, Ryan
Surprisingly, due to the structure of the proposed policies, we prove that for a subset of pull policies, the polynomial $E_i$ increases monotonically  with \psuccess. In this case, obtaining a lower bound on the end-to-end reliability only requires evaluating $E_i(P_s = P_m)$, which is both elegant and effective. %computationally-efficient. 

\textbf{Evaluation:}
We demonstrate the effectiveness of dynamic policies through testbed measurements and simulations. 
The results presented in Section \ref{sec:experiments} show that the developed dynamic policies significantly outperform traditional scheduling mechanisms. 
Through testbed experiments we show that policies can dynamically adapt in response to packet losses to provide links that have medium quality additional opportunities to transmit to improve reliability.
Simulation experiments indicate that for data collection workloads, policies provided a median improvement in real-time capacity of 2.6 times as well as a median reduction in response time of 2.4 times.%, effectively halving worst-case response time.


==> nc_fifo_proof.tex <==
% !TEX root = main.tex
\clearpage
\section{Appendix}
\label{sec:appendix}

\renewcommand{\psuccess}{\relax\ifmmode s\else $s$\xspace\fi}
\renewcommand{\pfailure}{\relax\ifmmode f \else $f$\xspace\fi}

\subsection{Proof of Theorem \ref{th:nonpreemptive-monotonic}}

\begin{proof}
Consider the execution on a non-preemptive pull policy on a single node $R$.
For simplicity, we will focus on the case when at most three instances $A_0$, $A_1$, and $A_2$ are active at a time; the same techniques may be used to extend for additional active instances. We use the notation $A_{i}$ instead of $J_i$ to emphasize that the active instances are ordered by the time when $R$ start executing them, rather than the priority of the instances. For brevity, we will use $P_s = s$ and $1 - P_s = f$.

Under these constraints, the node $R$ can be in one of four states --- $FFF$, $SFF$, $SSF$, and $SSS$ --- encoding the success of failures of executing instances $A_0$, $A_1$, and $A_2$ (in this order).
Note that, due to the preemptive nature of the policy, the system cannot in a state such as $FSS$ since instances $A_1$ and $A_2$ will not be executed unless $A_0$ has been previously successful (see Algorithm \ref{algo:runtime-behavior}). 



Let $S(t, \pfailure)$ be a vector representing the state of the system after executing the nonpreemptive poll policy for several slots.
Without loss of generality, consider that $S(t, \pfailure)$  has the form:

$S(t, \pfailure) = [P_{FFF}(t, \pfailure), P_{SFF}(t, \pfailure), P_{SSF}(t, \pfailure), P_{SSS}(t, \pfailure)]$


%\begin{displaymath}
%S(t, \pfailure) = 
%\begin{pmatrix} 
%P_{FFF}(t, \pfailure) \\
%P_{SFF}(t, \pfailure) \\  
%P_{SSF}(t, \pfailure) \\
%P_{SSS}(t, \pfailure)
%\end{pmatrix}^{T}
%\end{displaymath} 

\noindent Note that $S(t, \pfailure)$ is also parameterized by \pfailure instead of \psuccess as it leads to simpler expressions. Given $S(t, \pfailure)$, the reliability of each instance is:

\begin{IEEEeqnarray}{rCl}
E_0(t, \pfailure) & = & P_{SFF}(t, \pfailure) + P_{SSF}(t, \pfailure) + P_{SSS}(t, \pfailure) \nonumber \\
E_1(t, \pfailure) & = & P_{SSF}(t, \pfailure) + P_{SSS}(t, \pfailure) \nonumber \\
E_2(t, \pfailure) & = & P_{SSS}(t, \pfailure) \nonumber
\end{IEEEeqnarray}

In general, the possible configurations of active instances considered by $R$ at run-time are $(A_0) \subset (A_0, A_1) \subset (A_0, A_1, A_2)$ resulting in the execution of \pull{R}{$A_0$}, \pull{R}{$A_0, A_1$}, or \pull{R}{$A_0, A_1, A_2$}, respectively. 
In the following, we will focus on the execution of \pull{R}{$A_0, A_1, A_2$}; the other cases are similar. 

\begin{figure}
\centering
    \includegraphics[width=.5\linewidth]{figures/nc_one_step.pdf}
    \caption{MC describing the state updates for executing \pull{R}{$A_0, A_1, A_2$} }
    \label{fig:nc-nonpreemptive:mc}
\end{figure}

The execution of  \pull{R}{$A_0, A_1, A_2$} is described by the MC shown in Figure \ref{fig:nc-nonpreemptive:mc}.
The structure of the MC reflects that the instances in the service list are executed in order only of the all the previous instances have been successful.
Accordingly, if none of the instances have been successful, the system is in state $FFF$.
In this case, the first instance $A_0$ will be executed and the system may either stay in $FFF$ or transition to $SFF$ depending on the outcome of the \pullop.
Note that in the case instances have already been successful i.e., the system is in state $SSS$ no instances will be executed and the system remains in this state with likelihood of 1.  
After the execution of  \pull{R}{$A_0, A_1, A_2$} the state $S(t+1)$ is:

\begin{displaymath}
S(t + 1, \pfailure) = 
\begin{pmatrix} 
\pfailure P_{FFF}(t, \pfailure)\\ 
(1 - \pfailure)P_{FFF} + fP_{SFF}(t, \pfailure)\\ 
(1 - \pfailure) P_{SFF}(t, \pfailure) + \pfailure P_{SSF}(t, \pfailure)\\ 
(1 - \pfailure) P_{SSF}(t, \pfailure) + P_{SSS}(t, \pfailure)
\end{pmatrix}^{T}
\end{displaymath}

After substituting $P_{FFF}(t, \pfailure) = 1 - P_{SFF}(t, \pfailure) - P_{SSF}(t, \pfailure) - P_{SSS}(t, \pfailure)$, the end-to-end reliabilities are:
\begin{IEEEeqnarray}{rCl}
E_0(t+1, \pfailure) & = & (1 - \pfailure) + \pfailure (P_{SFF}(t, \pfailure) + P_{SSF}(t, \pfailure) + P_{SSS}(t, \pfailure)) \nonumber \\
               &  = & (1 - \pfailure) + \pfailure E_0(t, \pfailure) \nonumber \\
E_1(t+1, \pfailure) & = & (1-\pfailure) P_{SFF}(t, \pfailure) + P_{SSF}(t, \pfailure) + P_{SSS}(t, \pfailure) \nonumber \\
                & = & (1-\pfailure) P_{SFF}(t, \pfailure) + E_1(t, \pfailure) \nonumber \\ 
E_2(t+1, \pfailure) & = & (1 - \pfailure)  P_{SSF}(t, \pfailure) + P_{SSS}(t, \pfailure) \nonumber \\
	       & = & (1 - \pfailure)  P_{SSF}(t, \pfailure) + E_2(t, \pfailure) \nonumber
\end{IEEEeqnarray}

We will use an inductive argument to prove the end-to-end reliability of flows is monotonic when using nonpreemptive pull policies.
The base case of the induction when $S(t) = [1, 0, 0,0]$ indicating the none of the active instances have been successful can be easily verified. Let's focus on the inductive step. We what to show that if $E_i(t, \pfailure)$ is monotonically decreasing with \pfailure (and increasing with \psuccess),
then $E_i(t+1)$ is decreasing monotonically with \pfailure (and increasing with \psuccess).
To prove these functions are monotonically decreasing it is sufficient to prove their derivatives $E'_i(t+1)=\frac{\partial E_i(t+1)}{\partial\pfailure}$ are negative for all $\pfailure \in (0, 1)$ and $i = \{0,1,2\}$.

By differentiating $E_0(t+1, \pfailure)$, we obtain:

\begin{displaymath}
E'_0(t+1, \pfailure) = (-1 + E_0(t, \pfailure)) + (\pfailure E'_0(t, \pfailure)) \le 0
\end{displaymath}

\noindent The term $- 1 + E_0(t, \pfailure) \le  0$ since $E_0(t, \pfailure) \le 1$.
Similarly, the term $\pfailure E'_0(t, \pfailure) \le 0$  since $\pfailure \in (0, 1)$ and $E'_0(t, \pfailure) \le 0$ by the inductive assumption. Therefore,  $E_0(t+1, \pfailure) \le 0$

Next, we  will prove that $E_1'(t + 1, \pfailure) \le 0$. By differentiating, we obtain:
\begin{IEEEeqnarray}{rCl}
E'_1(t+1, \pfailure) & = & -P_{SFF}(t, \pfailure) + (1-\pfailure)P'_{SFF}(t, \pfailure)  \nonumber \\
                               & &+ P'_{SSF}(t, \pfailure) + P'_{SSS}(t, \pfailure) \nonumber \\
                               & = & -P_{SFF}(t, \pfailure) + (1-\pfailure)P'_{SFF}(t, \pfailure) + E'_1(t, \pfailure) \nonumber
\end{IEEEeqnarray}
\noindent We want to prove, $E'_1(t+1, \pfailure) \le 0$. By the inductive hypothesis, we know that $E'_0(t, \pfailure) \le 0$. 
Lets put the inequation in a more convenient form:
\begin{IEEEeqnarray}{rCl}
E'_0(t, \pfailure) & \le & 0  \nonumber \\
P'_{SFF}(t, \pfailure) + P'_{SSF}(t, \pfailure) + P'_{SSS}(t, \pfailure)  & \le & 0 \nonumber \\
P'_{SFF}(t, \pfailure) + E'_1(t, \pfailure)  & \le & 0 \nonumber \\
P'_{SFF}(t, \pfailure)  & \le & -E'_1(t, \pfailure)  \nonumber \\
(1-\pfailure) P'_{SFF}(t, \pfailure)  & \le & -(1-\pfailure) E'_1(t, \pfailure)  \nonumber 
\end{IEEEeqnarray}

\noindent By substituting in $E'_1(t +1, \pfailure)$, we obtain:
\begin{IEEEeqnarray}{rCl}
E'_1(t+1, \pfailure) & = & -P_{SFF}(t, \pfailure) + (1-\pfailure)P'_{SFF}(t, \pfailure) + E'_1(t, \pfailure) \nonumber \\
                              & \le &  -P_{SFF}(t, \pfailure) -(1-\pfailure) E'_1(t) + E'_1(t, \pfailure) \nonumber \\
                              & \le &  -P_{SFF}(t, \pfailure) + \pfailure E'_1(t)  \nonumber \\
                              & \le & 0 \nonumber
\end{IEEEeqnarray}
\noindent  A similar argument holds for $E'_0(t + 1) \le 0$.


We have shown that from an arbitrary state $S(t, \psuccess)$ in which the end-to-end reliability is monotonically increasing with \psuccess (and decreasing with \pfailure), we reach a next state $S(t+1, \psuccess)$ in which the end-to-end reliabilities remain monotonic.
Therefore, via induction, the end-to-end reliability of nonpreemptive policies always increases monotonically with \psuccess.
 








% \begin{figure}
% \small
% \centering
% \begin{subfigure}[b]{\linewidth}
% \vskip 0pt
% \centering
% \begin{tikzpicture}[shorten >=2pt,node distance=1.8cm,on grid,auto] 
%   \node[state,initial] (fff)   {FFF}; 
%   \node[state,accepting] (sff)  [right=of fff] {SFF}; 
%   \node[state,accepting] (ssf)  [right=of sff] {SSF};
%   \node[state,accepting] (sss)  [right=of ssf] {SSS};
%     \draw[->]
%     (fff) edge[above] node {\psuccess} (sff)
%     (sff) edge[above] node {\psuccess} (ssf)
%     (ssf) edge[above] node {\psuccess} (sss)
    
%     (fff) edge[loop above] node {\pfailure} (fff)
%     (sff) edge[loop above] node {\pfailure} (sff)
%     (ssf) edge[loop above] node {\pfailure} (ssf)
%     (sss) edge[loop above] node {1} (sss)
%     ;
% \end{tikzpicture}
% \caption{MC describing the execution of the policy \policy}
% \label{fig:nonpreemptive-mc}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
% \vskip 0pt
% \centering
% \begin{tikzpicture}[shorten >=2pt,node distance=1.8cm,on grid,auto] 
%   \node[state] (fff1)   {FFF}; 
%   \node[state] (sff1)  [below=of fff1] {SFF}; 
%   \node[state] (ssf1)  [below=of sff1] {SSF};
%   \node[state] (sss1)  [below=of ssf1] {SSS};
   
%   \node[state] (fff2)  [right=of fff1] {FFF}; 
%   \node[state] (sff2)  [right=of sff1] {SFF}; 
%   \node[state] (ssf2)  [right=of ssf1] {SSF};
%   \node[state] (sss2)  [right=of sss1] {SSS};
   
%     \draw[->]
%     (fff1) edge[above] node {\psuccess} (sff2)
%     (sff1) edge[above] node {\psuccess} (ssf2)
%     (ssf1) edge[above] node {\psuccess} (sss2)
    
%     (fff1) edge[above] node {\pfailure} (fff2)
%     (sff1) edge[above] node {\pfailure} (sff2)
%     (ssf1) edge[above] node {\pfailure} (ssf2)
%     (sss1) edge[above] node {1} (sss2)
%     ;
% \end{tikzpicture}
% \caption{The MC unrolled for one step}
% \label{fig:nonpreemptive-mc-unrolled}

% \end{subfigure}
% \caption{belea}
% \end{figure}
\end{proof}

==> policy_builder.tex <==
% !TEX root = main.tex
\subsubsection{\pn Builder}
\label{sec:policy-builder}
The \builder determines the \pullops that will be assigned in a slot. 
In each slot, the \evaluator supplies the \builder with a list of released flows and their associated active links. 
The builder then determines a set of \pullops that maximizes the number of flows that are executed in the slot while enforcing the priorities of flows. 
It is important to note that the \builder does not use the state probabilities maintained by the \evaluator since this information is not necessary given the optimization objective.
%; this information is captured (partially) by the list of active links supplied by the \evaluator.



The optimization problem can be formulated as an Integer Linear Program (ILP).
The ILP includes three types of variables.
For each node $R$ ($R \in \nodes$), the variable $N_R$ ($N_R \in \{0, 1\}$) indicates whether $R$ is the coordinator of a \pullop.
For each released instance $J_i$, the variable $I_i$ ($I_i \in \{0, 1\}$) indicates whether its associated active link will be added to a service list.
Finally, variable $C_{R,ch}$ ($C_{R,ch} \in \{0, 1\}$) indicates whether $R$ will use channel $ch$ to communicate.
%The ILP solution determines the \pullops that will be assigned in the current slot as follows
The ILP solution is converted into a set of \pullops as follows:
for each node $R$ such that $N_R=1$, we add a \pullop that has $R$ as the coordinator and a service list with all instances $J_i$
where $I_i = 1$ and $R$ is the receiver of the active link of $J_i$.
%where $R$ as a destination (i.e., $dst(J_i) = R$) and $I_i = 1$.
The \pullop is assigned to the entry in the matrix for the current slot and the channel $ch$ for which $C_{R,ch}=1$.
%The channel of the \pullop is the channel $ch$ for which $C_{R,ch}=1$.



% \textbf{Preemptive Pull Policies:}
A well-formed policy must ensure that no transmission conflicts will be introduced at run-time.
Consider a \pullop that has $R$ as a coordinator and services instance $J_i$.
Let $(SR)$ be the active link of $J_i$, where $S=src(J_i)$ and $R=dst(J_i)$. 
If $J_i$ will be assigned in the current slot (i.e., $I_i = 1$), then $S$ cannot be a coordinator for any other instance since this would require $S$ to transmit and receive in the same slot.
We enforce this using the following constraint:



\begin{IEEEeqnarray}{c}
N_S \le (1 - I_i) ~~~~\forall I_i \in \mathcal{A}: ~~S=src(J_i) 
\label{eq:constraint-sender}
\end{IEEEeqnarray}

\noindent A similar constraint must also be included for the receiver $R$. 
If node $R$ is not a coordinator (i.e., $N_R = 0$), then $J_i$ cannot be assigned and $I_i = 0$.
Conversely, if $R$ is selected as a coordinator, instance $J_i$ may (or may not) be assigned (i.e., $I_i \le N_R = 1)$ depending on the objective of the optimization, which we will discuss later in this section.
These aspects are captured by the following constraint:

\begin{IEEEeqnarray}{c}
I_i \le N_R   ~~~~\forall I_i \in \mathcal{A}: ~~R=dst(J_i) 
\label{eq:constraint-receiver}
\end{IEEEeqnarray}

\input{th_wellformed.tex}

The above constraints avoid all transmission conflicts with one exception.
Consider the case when two instances $J_i$ and $J_j$ share the same sender but have different receivers.
% as depicted in Figure \ref{fig:common-sender}.
An assignment that respects constraints \ref{eq:constraint-sender} and \ref{eq:constraint-receiver} is for both instances to be assigned in the current slot (i.e., $I_i = I_j = 1$). 
However, this would result in a conflict, since the common sender can only transmit one packet in a slot.
To avoid this situation, we introduce the following constraint:


\begin{IEEEeqnarray}{rCl}
 & I_i + I_j - 1 \le N_{S} & \label{eq:constraint-pairs}\\
 & \forall I_i, I_j \in \mathcal{A}: ~~S = src(J_i) = src(J_j) ~~\& ~~dst(J_i) \ne dst(J_j) & \nonumber
\end{IEEEeqnarray}

\begin{theorem}
    Constraints \ref{eq:constraint-sender}, \ref{eq:constraint-receiver}, and \ref{eq:constraint-pairs} ensure that the execution of \pullops will result in no node receiving or transmitting more than once in a time slot.
    \label{th:partially-wellformed}
\end{theorem}


\input{proof_wellformed.tex}

The next set of constraints ensures that each \pullop is assigned a unique channel.  
We accomplish this by introducing $C_{R,ch}$ to indicate whether coordinator $R$ uses channel $ch$ ($ch = 1 \dots K$), where $K$ is the number of channels.
The selection of channels is subject to the constraints:

\begin{IEEEeqnarray}{c}
 \sum_{R \in \mathcal{V}}{C_{R,ch} } \le 1  ~~~ \forall ch \in 1 \dots K  \\
 \sum_{ch=1}^{K}{C_{R,ch}} = N_{R}
\end{IEEEeqnarray}

A requirement of the TLR model described in Section \ref{sec:reliability-model} is that coordinators must switch channels between \pullops to ensure independence between transmissions. We enforce this property by introducing additional constraints to prevent coordinators from using the same channel.

% if i is the highest priority then this is wrong since i will be given the lowest weight
To enforce the prioritization of instances, we set the optimization objective to be:
\begin{IEEEeqnarray}{c}
\sum_{i = 0}^{i < |\mathcal{A}|}{2^{|\mathcal{A}| - i} * I_i}
\end{IEEEeqnarray}

\noindent The objective function ensures that a flow $F_i$ will be assigned over lower priority flows unless there is a higher priority flow with a conflict with $F_i$.

\subsubsection{\pn Builder}
The \builder determines the \pullops that will be assigned in a slot. 
In each slot, the \evaluator supplies the \builder with a list of released flows and their associated active links. 
The builder then determines a set of \pullops that maximizes the number of flows that are executed in the slot while enforcing the priorities of flows. 
It is important to note that the \builder does not use the state probabilities maintained by the \evaluator since this information is not necessary given the optimization objective.
%; this information is captured (partially) by the list of active links supplied by the \evaluator.



The optimization problem can be formulated as an Integer Linear Program (ILP).
The ILP includes three types of variables.
For each node $R$ ($R \in \nodes$), the variable $N_R$ ($N_R \in \{0, 1\}$) indicates whether $R$ is the coordinator of a \pullop.
For each released instance $J_i$, the variable $I_i$ ($I_i \in \{0, 1\}$) indicates whether its associated active link will be added to a service list.
Finally, variable $C_{R,ch}$ ($C_{R,ch} \in \{0, 1\}$) indicates whether $R$ will use channel $ch$ to communicate.
%The ILP solution determines the \pullops that will be assigned in the current slot as follows
The ILP solution is converted into a set of \pullops as follows:
for each node $R$ such that $N_R=1$, we add a \pullop that has $R$ as the coordinator and a service list with all instances $J_i$
where $I_i = 1$ and $R$ is the receiver of the active link of $J_i$.
%where $R$ as a destination (i.e., $dst(J_i) = R$) and $I_i = 1$.
The \pullop is assigned to the entry in the matrix for the current slot and the channel $ch$ for which $C_{R,ch}=1$.
%The channel of the \pullop is the channel $ch$ for which $C_{R,ch}=1$.



% \textbf{Preemptive Pull Policies:}
A well-formed policy must ensure that no transmission conflicts will be introduced at run-time.
Consider a \pullop that has $R$ as a coordinator and services instance $J_i$.
Let $(SR)$ be the active link of $J_i$, where $S=src(J_i)$ and $R=dst(J_i)$. 
If $J_i$ will be assigned in the current slot (i.e., $I_i = 1$), then $S$ cannot be a coordinator for any other instance since this would require $S$ to transmit and receive in the same slot.
We enforce this using the following constraint:



\begin{IEEEeqnarray}{c}
N_S \le (1 - I_i) ~~~~\forall I_i \in \mathcal{A}: ~~S=src(J_i) 
\label{eq:constraint-sender}
\end{IEEEeqnarray}

\noindent A similar constraint must also be included for the receiver $R$. 
If node $R$ is not a coordinator (i.e., $N_R = 0$), then $J_i$ cannot be assigned and $I_i = 0$.
Conversely, if $R$ is selected as a coordinator, instance $J_i$ may (or may not) be assigned (i.e., $I_i \le N_R = 1)$ depending on the objective of the optimization, which we will discuss later in this section.
These aspects are captured by the following constraint:

\begin{IEEEeqnarray}{c}
I_i \le N_R   ~~~~\forall I_i \in \mathcal{A}: ~~R=dst(J_i) 
\label{eq:constraint-receiver}
\end{IEEEeqnarray}

\input{th_wellformed.tex}

The above constraints avoid all transmission conflicts with one exception.
Consider the case when two instances $J_i$ and $J_j$ share the same sender but have different receivers.
% as depicted in Figure \ref{fig:common-sender}.
An assignment that respects constraints \ref{eq:constraint-sender} and \ref{eq:constraint-receiver} is for both instances to be assigned in the current slot (i.e., $I_i = I_j = 1$). 
However, this would result in a conflict, since the common sender can only transmit one packet in a slot.
To avoid this situation, we introduce the following constraint:


\begin{IEEEeqnarray}{rCl}
 & I_i + I_j - 1 \le N_{S} & \label{eq:constraint-pairs}\\
 & \forall I_i, I_j \in \mathcal{A}: ~~S = src(J_i) = src(J_j) ~~\& ~~dst(J_i) \ne dst(J_j) & \nonumber
\end{IEEEeqnarray}

\begin{theorem}
    Constraints \ref{eq:constraint-sender}, \ref{eq:constraint-receiver}, and \ref{eq:constraint-pairs} ensure that the execution of \pullops will result in no node receiving or transmitting more than once in a time slot.
    \label{th:partially-wellformed}
\end{theorem}


\input{proof_wellformed.tex}

The next set of constraints ensures that each \pullop is assigned a unique channel.  
We accomplish this by introducing $C_{R,ch}$ to indicate whether coordinator $R$ uses channel $ch$ ($ch = 1 \dots K$), where $K$ is the number of channels.
The selection of channels is subject to the constraints:

\begin{IEEEeqnarray}{c}
 \sum_{R \in \mathcal{V}}{C_{R,ch} } \le 1  ~~~ \forall ch \in 1 \dots K  \\
 \sum_{ch=1}^{K}{C_{R,ch}} = N_{R}
\end{IEEEeqnarray}

A requirement of the TLR model described in Section \ref{sec:reliability-model} is that coordinators must switch channels between \pullops to ensure independence between transmissions. We enforce this property by introducing additional constraints to prevent coordinators from using the same channel.

% if i is the highest priority then this is wrong since i will be given the lowest weight
To enforce the prioritization of instances, we set the optimization objective to be:
\begin{IEEEeqnarray}{c}
\sum_{i = 0}^{i < |\mathcal{A}|}{2^{|\mathcal{A}| - i} * I_i}
\end{IEEEeqnarray}

\noindent The objective function ensures that a flow $F_i$ will be assigned over lower priority flows unless there is a higher priority flow with a conflict with $F_i$.

% \textbf{Non-Preemptive Pull Policies:}
% The constraints defined so far allow us to construct \emph{preemptive pull policies}, where the execution of lower priority instances is preempted by that of higher priority instances.
% We can also build \emph{non-preemptive pull policies} that have the additional constraint that once an instance has started being executed by a node, it cannot be preempted by an instance with the same coordinator. 
% As detailed in the next section, the end-to-end reliability of flows may be computed in a simpler manner when non-preemptive policies are used.
% Non-preemptive policies can be constructed by incorporating additional constraints into the ILP.
% We accomplish this by tracking when instances start their execution at each node $R$ in a $exec[R]$ FIFO queue.
% % this still isn't right.  Consider instances I1 and I2 that are in the exec queue.  Then I0 preempts I1 and I1 (this constraint allows this) and is added to exec.  The order of exec may now be messed up.  In the actual code this is the constraint that I use "for all I in exec[R] I = N_R".  This way the I's in exec will only be suspended if it due to a conflict on one of the senders.  Moreover, there is no risk that the exec list will be messed up since no instance will be added that uses it unless all the other instances are scheduled.  I then make sure things are ordered correctly after the ILP returns the result.
% An instance is added to $exec[R]$ when it is first included in the service list of a \pullop on node $R$ and removed when the \evaluator determines it has met its end-to-end reliability.
% We impose the constraint that $R$ can be a coordinator (i.e., $N_R=1$) if and only if \emph{all} instances in the $exec[R]$ set will be executed:

% \begin{equation}
%     I_{i} = N_R~~~~~~~~~\forall R \in \nodes~\textrm{and}~\forall I_i \in exec[R]
% \end{equation}





